Elixir: A system to enhance data quality for multiple analytics on a video stream

IoT sensors, especially video cameras, are ubiquitously deployed around the world to perform a variety of computer vision tasks in several verticals including retail, healthcare, safety and security, transportation, manufacturing, etc. To amortize their high deployment effort and cost, it is desirable to perform multiple video analytics tasks, which we refer to as Analytical Units (AUs), off the video feed coming out of every camera. In this paper, we first show that in a multi-AU setting, changing the camera setting has disproportionate impact on different AUs performance. In particular, the optimal setting for one AU may severely degrade the performance for another AU, and further the impact on different AUs varies as the environmental condition changes. We then present Elixir, a system to enhance the video stream quality for multiple analytics on a video stream. Elixir leverages Multi-Objective Reinforcement Learning (MORL), where the RL agent caters to the objectives from different AUs and adjusts the camera setting to simultaneously enhance the performance of all AUs. To define the multiple objectives in MORL, we develop new AU-specific quality estimator values for each individual AU. We evaluate Elixir through real-world experiments on a testbed with three cameras deployed next to each other (overlooking a large enterprise parking lot) running Elixir and two baseline approaches, respectively. Elixir correctly detects 7.1% (22,068) and 5.0% (15,731) more cars, 94% (551) and 72% (478) more faces, and 670.4% (4975) and 158.6% (3507) more persons than the default-setting and time-sharing approaches, respectively. It also detects 115 license plates, far more than the time-sharing approach (7) and the default setting (0).

==> common_and_digital_transformation.tex <==
%\subsection{After-capture transformation with parameter tuning}
%\subsection{Further improvement over \approach}
%\label{subsec:discussion_common_param_tuning}

%\begin{table}[tb]
%\centering
%\begin{tabular}{|c|c|c|}
%    \hline
%     Camera Setting & PD accuracy & FD accuracy \\
%     & mAP$_{PD}$(\%) & mAP$_{FD}$(\%)  \\
%     & (DAY) & (NIGHT) \\
%    \hline
%    \emph{Common-optimal}  & 91.7 & 48.8 \\
%    \hline
%    \emph{Common-optimal}  & 98.8 & 50.0\\
%    \emph{+ AU-specific Tx} & \\
%    \hline
%\end{tabular}
%\caption{Improvement over \approach}
%\label{tab:further_improvement}
% \vspace{-0.3in}
%\end{table}
 
%In ~\secref{subsec:optimal_settings_conflict}, as shown in ~\tabref{tab:night-overall}, we saw that FD achieves 48.8\% accuracy using common-optimal setting, while the highest achieved accuracy using FD-optimal setting is 50\%. Also, for PD, as shown in ~\tabref{tab:day-overall} the accuracy achieved using common-optimal setting is 91.7\% while the highest achieved accuracy using PD-optimal setting is 99.36\%. Thus, there is a gap in the highest possible accuracy and the one achieved by common-optimal setting. In this section, we show that it is possible to reduce this gap i.e. boost the accuracy further, by applying AU-specific digital transformation on the camera feed for each AU, after \approach\ tunes the camera settings to common-optimal setting.

%For this study, on the frame captured with ``common-optimal" setting discussed in ~\secref{subsec:optimal_settings_conflict}, we exhaustively apply different digital transformations by using PIL library ~\textcolor{blue}{[add citation]} and run these frames through
%the yolov5 object detection model for PD and retinaNet face detection model for FD
%PD and FD AUs. We then choose the digital transformation that provides the highest accuracy. ~\tabref{tab:further_improvement} shows that the accuracy for PD is further boosted from 91.7\% to 98.8\% and accuracy for FD is further boosted from 48.8\% to 50\%. \textit{Thus, it is indeed possible to further improve the accuracy of the AUs by applying AU-specific digital transformations on the frame, after \approach\ tunes the camera settings to common-optimal settings that works well for multiple AUs.} Note that in ~\cite{paul2021camtuner}, it is shown that directly applying digital transformation on frames does not improve accuracy, if the frame capture itself is of ``poor" quality. Therefore, we did not directly apply digital transformations on the frames captured with default camera settings, rather we first let \approach\ tune the camera settings to common-optimal setting in order to enhance data quality, and then apply digital transformation on them. This ``common-optimal + AU-specific digital transformation" gives further improvement in accuracy over \approach.

%~\tabref{tab:overall-optimal-discuss} shows the impact of cumulative FD and PD accuracy improvement after applying the best post-capture data transformation for \emph{NIGHT} and \emph{DAY} environment.  

%Although camera parameter tuning provides superior performance over post-capture image transformation. In a multi-AU scenario, we here investigate whether the overall VAP performance can further be boosted by applying each AU-specific post-capture image transformation on the frame captured with common-optimal camera setting based on the combined perception of multiple AUs. We here extend the experiment presented in~\secref{subsec:optimal_setting_exists} to find out the impact of post-capture transformation on top of common-optimal camera setting. Using PIL library~\cite{}, we exhaustively apply different post-capture data transformation on the captured frame and pass them through the yolov5 object detection model for person detection (PD) and retinaNet face detection (FD) model. ~\tabref{tab:overall-optimal-discuss} shows the impact of cumulative FD and PD accuracy improvement after applying the best post-capture data transformation for \emph{NIGHT} and \emph{DAY} environment.  

%\begin{table}[h!]
%\begin{subtable}[h!]{0.45\textwidth}
%\centering
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|}
%    \hline
%    Camera Setting & FD accuracy & PD accuracy & improv\\
%    & mAP$_{FD}$(\%) & mAP$_{PD}$(\%) & (\%) \\
%    \hline
%    \emph{Default} & 38.9 &  58.3 & +0\\
%    \hline
%    \emph{Default} & 38.9 & 58.3 & +0 \\
%    \emph{+ AU-specific Tx} &  &  & \\
%    \hline
%    \emph{Common-optimal} & 48.8 & 83.3 & +35.9\\
%    \hline
%    \emph{Common-optimal} & 50.0 & 83.3 & +37.1 \\
%    \emph{+ AU-specific Tx} &  &  & \\
%    \hline
%\end{tabular}}
%\caption{NIGHT}
%\label{tab:night-overall-discuss}
%\end{subtable}

%\begin{subtable}[h!]{0.45\textwidth}
%\centering
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|}
%    \hline
%     Camera Setting & FD accuracy & PD accuracy &  improv\\
%    & mAP$_{FD}$(\%) & mAP$_{PD}$(\%) & (\%) \\
%    \hline
%    Default & 82.6 & 90.9 &  +0 \\
%    \hline
%    \emph{Default} &  98.7 & 91.7 &  +9.7 \\
%    \emph{+ AU-specific Tx} &  &  & \\
%    \hline
%    \emph{Common-optimal} & 100.0 & 91.7 &  +10.5 \\
%    \hline
%    \emph{Common-optimal} & 100.0 & 98.8 &  +14.6\\
%    \emph{+ AU-specific TX} & & & \\
%    \hline
%\end{tabular}}
%\caption{DAY}
%\label{tab:day-overall-discuss}
%\end{subtable}
%\caption{Overall Optimal Setting and PostProcessing for Multiple AUs}
%\label{tab:overall-optimal-discuss}
% \vspace{-0.3in}
%\end{table}


%\begin{figure}
%    \centering

        % \includegraphics[width=\textwidth]{figs/impact_all_2.pdf}
%        \includegraphics[width=0.5\textwidth]{figs/multiAU_setup.PNG}
%        \caption{Single Camera Setting and Multiple Virtual Camera Settings for Multiple AU setup}
%        \label{fig:mulAU_setup}
%\vspace{-0.1in}
%\end{figure}

%~\tabref{tab:overall-optimal-discuss} also indicates that applying different post-capture digital transformation adapting to various AUs can further enhance the AU performance after the camera is tuned at a common-optimal camera setting. 

==> exp_setup.tex <==

\subsubsection{Experimental Setup}
\label{subsubsec:expsetup}

Comparing different policy aggregation strategies in a real-world deployment is difficult because (1) We need multiple co-located cameras each for one policy which look at the identical scene from the same angle; (2) furthermore, in a real-world deployment, the captured scenes do not have the ground-truth to measure the AU accuracy.
%
To overcome the above challenge, we loop a pre-recorded (original) 2-minute video snippet (a customer video captured at the entrance of the enterprise building as captured in~\secref{subsec:optimal_setting_across_au}) labeled with ground-truth through virtual camera (VC) as presented in~\cite{paul2021camtuner} -- VC is used here not for RL training but for generating {\em augmented} input videos that emulate different environmental changes to be fed into the different VAPs each for one policy aggregation strategy.  In particular, we gradually change the VC model parameters (\ie post-capture digital transformations) to simulate the changes that happen during the day as the Sun changes its position and finally sets, and we ensure (through manual inspection) that same ground-truths are carried over in the VC generated videos from the original video.

There are two possible approaches to evaluate, as follows 

\textbf{(Approach 1)} We then project these VC-generated videos on a monitor screen in front of a real camera, and run each of these multiple VAPs (each for one policy aggregation strategy) in turn. We set the camera parameters based on current scene and compute the accuracy with respect to the ground-truth. 
%sources of accuracy loss
\emph{Since, video frames played on the monitor screen already undergo several augmentation (information loss) by VC thus changing the camera settings and capturing the modified frame can suffer from accuracy loss. Along with that, pre-recorded video frames can also go through distortions due to projection}.


\textbf{(Approach 2)} We loop through VC-generated videos, and run each of the three VAPs in turn. Each VAP selects a specific image augmentation parameter and applies that on to the original pre-recorded video frames (captured under default setting). We then compute the accuracy of the generated video frame with respect to the ground-truth. 

To reduce distortion due to projection error, we opt for the approach 2 to evaluate different VAPs under controlled experimental setup.


We use approach 2 to evaluate the impact of different policy choices for MORL agent in \approach\ design. We evaluate four AU's accuracy (\ie true-positive detection count) improvement for four 2-minute video segments randomly selected from the VC-generated videos  consisting of 1000 frames each and each video segment corresponds to a different hour that is separated by 2 hours apart. The original 2-minute video snippet is the proprietary video captured with default camera setting as mentioned in~\secref{subsec:optimal_setting_across_au}. We then use post-capture digital transformation to change the capture hour of the original video using VC~\cite{paul2021camtuner}. Using the labeled ground-truth~\footnote{We ensure that the ground-truth annotation performed for original video should remain intact for VC-generated videos as well}, we evaluate how \approach-tuned image augmentation parameters improve the total TP detection count~\footnote{A detection is considered as true-positive (TP) when the class labels both for predicted and ground-truth bounding box are the same and IoU (intersection over union) between them is atleast 0.7} (considering all four AUs together) than the default video, as shown in~\figref{fig:policy_impact}. 

\begin{figure}
    \centering
        \includegraphics[width=0.495\textwidth]{figs/policy_impact_1.pdf}
        \caption{Impact of different MORL policies on cumulative true-positive detection count improvement over default setting considering four different analytics \ie FD, PD, CD, LPD (under controlled experimental setup).}
        \label{fig:policy_impact}
\end{figure}

~\figref{fig:policy_impact} shows that \emph{policy 3} to combine 4 different Q-values (\ie each for one AU) into the aggregate Q-table performs the best compared to the other two aggregation strategies considering all 4 different time segments. Next, we use \emph{policy 3} to combine Q-values for different objectives (each for one AU) in our real-world \approach\ performance evaluation. 

==> optimal_setting_within_AU.tex <==
\subsection{Optimal camera setting varies within an AU}
\label{subsec:optimal_setting_within_au}
%\begin{figure}[tb]
%\begin{subfigure}[]{0.5\linewidth}
%\centering
%    \includegraphics[height=0.85 in]{figs/day.jpg}
%    \caption{DAY}
%    \label{fig:day_capture}
%\end{subfigure}%
%\begin{subfigure}[]{0.5\linewidth}
%\centering
%    \includegraphics[height=0.85 in]{figs/night.jpg}
%    \caption{NIGHT}
%    \label{fig:night_capture}
%\end{subfigure}
% \caption{Camera captures under different environment}
%  \label{fig:day-night-capture}
% \vspace{-0.2in}
%\end{figure}

\begin{table}[tb]
\centering
\begin{tabular}{|c|c|c|}
    \hline
    AU &  Optimal camera setting & Optimal camera setting \\
       & [brightness, contrast, & [brightness, contrast,  \\
       &  color, sharpness] &  color, sharpness] \\
       & \textbf{(Day time)}  & \textbf{(Night time)} \\
    \hline
    PD & [40,90,60,100] & [80,90,70,100]  \\
    \hline
    FD & [60,40,90,90] & [80,90,60,80]  \\
    \hline
\end{tabular}
\caption{Optimal camera setting for different environment}
\label{tab:optimal_camera_setting}
 \vspace{-0.3in}
\end{table}

\textcolor{blue}{Acknowledge CamTuner shows similar results ..}
In this section we show that for an AU,  optimal camera settings are not the same all the time and varies depending on the environmental conditions. In order to study if the optimal camera settings remain the same or vary depending on environmental conditions, we print 12 different person cutouts obtained from COCO dataset~\cite{lin2014microsoft} and place them in front of a real camera. Next, we use two sources of light, one of them is always turned ON and the other is turned ON to simulate DAY condition and the turned OFF to simulate NIGHT condition. 
%The observed scene by the camera in default camera settings is shown in ~\figref{fig:day-night-capture} for DAY and NIGHT conditions. 
By using two sources of light, we can change the environmental conditions around the camera by just turning one source of light ON or OFF. 

To study if the optimal camera settings under these two conditions is the same or not, we use two AUs i.e. Person detection (PD) which uses EfficientDet-v0~\cite{tan2020efficientdet} model and face detection (FD) AU which uses RetinaNet~\cite{deng2019retinaface} model. For each of the conditions i.e. DAY and NIGHT, we modify the four camera settings i.e. brightness, contrast, color and sharpness ranging from 0 to 100 in steps of 10, and capture the image from the camera for each of the ``modified" setting. In total, we obtain $\approx$14.6K (11$^4$) different images and on these images we run PD and FD. ~\tabref{tab:optimal_camera_setting} shows the optimal camera setting i.e. the one that gives highest AU accuracy, which is measured as a combination of mAP and true-positive IoU (the one with highest mAP and among same top mAPs, the one with hightest IoU). We observe that for PD, during the day time, the optimal camera settings is: brightness: 40, contrast: 90, color: 60 and sharpness: 100, while during night time, the optimal camera settings is: brightness: 80, contrast: 90, color: 70 and sharpness: 100. These optimal camera settings for same AU (PD) are different for day and night conditions. Similar observation is seen for FD as well, as shown in ~\tabref{tab:optimal_camera_setting}. \textit{Thus, optimal camera settings vary even for a single AU depending on the environmental conditions.}





%{\textbf{Impact.}} To observe the impact of camera setting on various AUs as well as for different environments, we have printed 12 different person cutouts obtained from COCO dataset~\cite{} and placed in front of a real camera. We have used EfficientDet-v0~\cite{} as person-detection AU and RetinaNet~\cite{} as face-detection AU and observe the impact on each of these AUs individually under \emph{DAY} and \emph{NIGHT} condition simulated inside our lab. In our setup, we use two light sources and keep one of them always \textit{ON}, while the other one is manually turned \emph{ON} or {OFF}. \emph{DAY} condition is simulated when both the light bulbs are turned \emph{ON}, appeared as bright. While keeping only one light bulb \emph{ON} emulates low-light condition, thereby simulating \emph{NIGHT} condition. For each of these conditions, we vary four image appearance camera settings (used in ~\cite{paul2021camtuner}) i.e., brightness, contrast, sharpness and color saturation ranging from 0 to 100 at a step of 10. ~\figref{fig:day-night-capture} shows the images captured under default camera setting for \emph{DAY} and \emph{NIGHT} condition. We obtained 14641 different images for various camera parameter settings for each of these environments and obtained the analytical quality (AQ) metric (i.e., combination of mAP and true-positive IoU explained in ~\secref{sec:motivation}). 



==> policy.tex <==
\subsection{Impact of different aggregation policies}
\label{subsec:policy}
The optimal policy in a multi-objective setting depends on the relative preferences among competing criteria \ie different downstream AUs' perception. Aggregation of multiple competing objectives is the key to opportunistically prioritize different downstream analytic tasks in a  multi-objective reinforcement learning (MORL) setup. We try out three different aggregation strategies for MORL, which are as follows:
\begin{enumerate}
    \item \textbf{Policy 1}: It provides equal weightage to all downstream task. It averages the individual Q-values obtained for each AU. 
    \begin{equation*}
        Q_{agg} = \sum_{i \in AU} Q_{i}[s,a] / count_{AU}
    \end{equation*}
        \item \textbf{Policy 2}: It uses pre-defined non-uniform priorities (\ie weightages) based on granularity of the downstream task. We used the insight of face-detection and license plate detection is much more fine-grained than person and car detection. We assign priority values for four AUs \ie $p_{FD}$, $p_{LPD}$, $p_{PD}$, $p_{CD}$ as 3, 2, 1,1 respectively. 
    \begin{equation*}
        Q_{agg} = \sum_{i \in AU} (p_{i} * Q_{i}[s,a])/\sum_i p_{i} 
    \end{equation*}
    
    \item \textbf{Policy 3}: Here the multiAU Q table is updated based on the maximum discounted reward (using bellman equation) corresponding to each downstream AU. Policy 3 ensures that the selected action is guaranteed to be optimal for at least one objective.
    %Under single-policy approach, here we use W-learning approach~\cite{humphrys1996action} where 
    \begin{equation*}
        Q_{agg} = \max_{i \in AU} Q_{i}[s,a]
        \end{equation*}
\end{enumerate}




==> post_processing.tex <==
\subsection{Camera parameter tuning vs after-capture transformation}
\label{subsec:post_processing}
Tuning the camera parameter directly affects the frame acquisition which is fundamentally different from digital transformation or image restoration applied after capturing the frame by the camera sensor.


\begin{table}[h!]
\begin{subtable}[h!]{0.45\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline
    Camera Setting & \multicolumn{2}{c|}{FD accuracy} & \multicolumn{2}{c|}{PD accuracy}\\
    & \multicolumn{2}{c|}{mAP(\%)} & \multicolumn{2}{c|}{mAP(\%)}\\
    \cline{2-5}
    & Default & Best-Tx & Default & Best-Tx \\
    \hline
    [90,10,100,50] & 0.0 & 0.0 & 0.0 & 0.0 \\
    \hline
    [10,20,70,100] & 4.17 & 33.33 & 16.67 & 76.83 \\
    \hline
    [10,100,40,100] & 8.33 & 33.33 & 25.0 & 70.0 \\
    \hline
    [80,10,30,100] & 48.81 & 50.0 & 83.33 & 83.33 \\
    \hline
\end{tabular}
\caption{NIGHT}
\label{tab:night-sub-optimal}
\end{subtable}

\begin{subtable}[h!]{0.45\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline
    Camera Setting & \multicolumn{2}{c|}{FD accuracy} & \multicolumn{2}{c|}{PD accuracy}\\
    & \multicolumn{2}{c|}{mAP(\%)} & \multicolumn{2}{c|}{mAP(\%)}\\
    \cline{2-5}
    & Default & Best-Tx & Default & Best-Tx \\
    \hline
    [100,10,10,30] & 0.0 & 0.0 & 0.0 & 0.0 \\
    \hline
    [90,100,20,60] & 16.07 & 25.0 & 33.33 & 41.67 \\
    \hline
    [80,100,90,100] & 45.83 & 56.48 & 66.67 & 75.0 \\
    \hline
    [40,100,30,60] & 100.0 & 100.0 & 91.67 & 98.81 \\
    \hline
\end{tabular}
\caption{DAY}
\label{tab:day-sub-optimal}
\end{subtable}
\caption{Parameter Tuning vs Post-processing across AUs}
\label{tab:sub-optimal-vs-pp}
 \vspace{-0.3in}
\end{table}

 While ~\tabref{tab:sub-optimal-vs-pp} shows that post-processing after frame acquisition can definitely improve the analytics accuracy but if the frame is captured with the suboptimal settings, shown in then post-processing can't improve the accuracy of the insights derived by AU. Camera setting adapting the external environmental condition always provide superior performance than applying any after-capture post-processing, also shown in the last row of ~\tabref{tab:sub-optimal-vs-pp} with the AU performance under optimal camera parameter settings for each environment. 









==> pre_recorded.tex <==
\subsubsection{Pre-recorded videos}
\label{subsec:optimal_setting_conflict_prerecorded_videos}
We saw in ~\secref{subsec:optimal_setting_conflict_real_cameras} that with real cameras, we can clearly see the conflict between AUs i.e. optimal setting for one AU degrades performance of another AU. In order to study this effect on pre-recorded videos as well, where we do not have the luxury to change real camera settings, we did a workaround where we apply digital transformation corresponding to the four camera settings i.e. brightness, contrast, color and sharpness, on the pre-recorded video and note the accuracy of the AUs after the digital transformation.

\begin{algorithm}[tb]
{ 
\small
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \SetKwProg{Fn}{Function}{\string:}{}
    \SetKwFunction{FmAP}{mAP}
  \SetKwFunction{FAU}{AU}
  \SetKwFunction{FAugment}{Augment}
  \SetKwFunction{Fbconf}{Find-Best-Conf}
  \SetKwFunction{FExtract}{ExtractFrames}
  
  \caption{Find optimal configuration for detection}
  \label{alg:det-conf-search}
  \Input{\begin{minipage}[t]{6.5cm}%
     Video-snippet ($vs$) and ground-truth ($gt$);
     
     configurations ($confs$)
   \end{minipage}
  }
  \Output{Find optimal configuration conf:<bright,contrast,color,sharpness>}
  frames $\leftarrow$ \FExtract($vs$) \\
  \For{$conf$ in $confs$}{
  \For{frame in frames}{
    $frame_{aug}$ $\leftarrow$ \FAugment(frame, $conf$);
    
    $dets$ $\leftarrow$ \FAU($frame_{aug}$);
    
    mAP, true-positive IoU $\leftarrow$ \FmAP($dets$, $gt$);
    }
    Get the average mAP and true-positive IoU for all frames
}
Sort $confs$ based on average mAP;

For same top-1 mAP $confs$, sort based on average true-positive IoU;

\KwRet{top-1 $conf$ from final sorted list}
}
\end{algorithm}

In order to find the optimal digital transformation configuration that works the best for any detection AU, we use the algorithm as shown in Algorithm~\ref{alg:det-conf-search}. Here for each frame in the video snippet, we apply different digital transformations one by one, measure the mAP and IoU, then average them across all the frames, and finally pick the one with top mAP (measured using pycocotools~\cite{pycoco}), and among the top mAP, pick the one with highest true-positive IoU~\footnote{bounding box prediction with IoU > 0.5 and with correct classification}.

\if 0
 \begin{algorithm}[tb]
{ 
\small
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \SetKwProg{Fn}{Function}{\string:}{}
    \SetKwFunction{FmAP}{mAP}
  \SetKwFunction{FAU}{AU}
  \SetKwFunction{FAugment}{Augment}
  \SetKwFunction{Fbconf}{Find-Optimal-Conf}
  \SetKwFunction{FExtract}{ExtractFrames}
  \SetKwFunction{FD}{FaceDetection}
  \SetKwFunction{FP}{PersonDetection}
  
  \caption{Impact of optimal configuration for one AU on another AU}
  \label{alg:impact-on-another}
  \Input{\begin{minipage}[t]{6.5cm}%
     Video-Snippet ($vs$) and ground-truth ($gt$); 
     person-detection AU ($PD$) and face-detection AU ($FD$);
    
   \end{minipage}
  }
  %\Output{Find conf:<bright,contrast,color,sharp> that provides best $AQ$ for detection}
  \Output{Find impact}

    optimal-conf-PD = \Fbconf(PD, $vs$, $gt$) \\
    optimal-conf-FD = \Fbconf(FD, $vs$, $gt$) \\
    diff $\leftarrow$ []
    
    frames $\leftarrow$ \FExtract(vs) \\
    \For{frame in frames}{
    $frame_{aug}^{pd}$ $\leftarrow$ \FAugment(frame, optimal-conf-PD);
    
    $frame_{aug}^{fd}$ $\leftarrow$ \FAugment(frame, optimal-conf-FD);
    
    $dets^{pd}$ $\leftarrow$ \FP($frame_{aug}^{fd}$);
    
    $dets^{fd}$ $\leftarrow$ \FD($frame_{aug}^{pd}$);
    
    mAP$_{optimal-conf-PD}$ $\leftarrow$ \FmAP($dets^{pd}$, $gt$);
    
    mAP$_{optimal-conf-FD}$ $\leftarrow$ \FmAP($dets^{fd}$, $gt$);
     
    diff.append(mAP$_{optimal-conf-FD}$ - mAP$_{optimal-conf-PD}$) 
    }
    
\KwRet{diff}
    
}
\end{algorithm}
\fi

In order to study the impact of applying optimal setting for one AU on another AU, 
%we follow Algorithm~\ref{alg:impact-on-another}, where 
we first apply digital transformation on the frames extracted from video-snippet with the two optimal configurations (obtained using Algorithm~\ref{alg:det-conf-search}) separately, then run FD on the frames which are digitally transformed with optimal settings for PD and vice versa, and measure the difference in accuracy for each frame. Finally, we measure the number of frames that undergo degradation due to the conflict.


\paragraph{\textbf{Public video datasets.}} 

\begin{figure}
\def\tabularxcolumn#1{m{#1}}
 \begin{tabularx}{\linewidth}{@{}cXX@{}}
 \begin{tabular}{cc}
 \subfloat[Olympics]{\includegraphics[width=4cm]{figs/olympics_cdf.pdf}\label{fig:olympics_cdf}}
 & \subfloat[HMDB]{\includegraphics[width=4cm]{figs/hmdb_cdf.pdf}\label{fig:rhmdb_cdf}
 }
 \end{tabular}
 \end{tabularx}
 \caption{Impact of best-configuration on another AU}
  \label{fig:impact-au}
 \end{figure}

\begin{table}[tb]
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline
    Video dataset &  \multicolumn{4}{c|} {Accuracy (mAP) degradation(\%)}\\
    \cline{2-5}
    & \multicolumn{2}{c|}{PD-optimal for FD} & \multicolumn{2}{c|}{FD-optimal for PD}\\
    & \multicolumn{2}{c|}{(Impact on FD)} & \multicolumn{2}{c|}{(Impact on PD)}\\
    \cline{2-3}\cline{4-5}
    & Max & Mean & Max & Mean \\
    \hline
    HMDB51 & 100.0 & 20.89 & 73.42 & 15.32 \\
    \hline
    Olympics & 100.0 & 52.72 & 57.69 & 22.49 \\
    \hline
\end{tabular}
\caption{Accuracy degradation in public video datasets}
\label{tab:public_dataset}
\end{table}

\begin{figure}
\def\tabularxcolumn#1{m{#1}}
 \begin{tabularx}{\linewidth}{@{}cXX@{}}
 \begin{tabular}{cc}
 \subfloat[FD with FD-optimal-setting]{\includegraphics[width=4cm]{figs/best_swing_baseball_13.jpg}\label{fig:olympics_cdf}}
 & \subfloat[FD with PD-optimal-setting]{\includegraphics[width=4cm]{figs/worst_swing_baseball_13.jpg}\label{fig:hmdb_cdf}
 } \\
 \subfloat[PD with FD-optimal-setting]{\includegraphics[width=4cm]{figs/worst_sword_exercise_47.jpg}\label{fig:olympics_cdf}}
 & \subfloat[PD with PD-optimal-setting]{\includegraphics[width=4cm]{figs/best_sword_exercise_47.jpg}
\label{fig:impact-pics}
 }

 \end{tabular}
 \end{tabularx}
 \caption{Impact of optimal-setting on PD and FD}
  \label{fig:impact-au-pics}
 \end{figure}

We chose 13 video snippets from HMDB dataset~\cite{Kuehne11} and 8 video snippets from Olympics dataset~\cite{niebles2010modeling} and applied various digital transformations on the frames and ran two different AUs i.e. person detection (PD) AU (which uses EfficientDet-v0~\cite{tan2020efficientdet}) and face detection (FD) AU (which uses RetinaNet~\cite{deng2019retinaface}). ~\figref{fig:impact-au} indicates the fraction of frames that undergo accuracy degradation for both PD and FD. Each point (x,y) in ~\figref{fig:impact-au} shows that (100-x)\% of video frames experience at least a mAP degradation of y\%. ~\tabref{tab:public_dataset} shows the mean and max accuracy degradation due to the conflict. ~\figref{fig:impact-au-pics} shows visual representation of the images under different optimal settings and when PD and FD are applied on them. We see that for PD, optimal setting endeavours to increase the contrast, which enhances the pixel intensity difference, which in turn increases the distinguishability of person in the frame. However, increasing contrast adds noise, which makes it difficult for FD to detect small fine-grained features in the faces.

\paragraph{\textbf{Proprietary customer video datasets.}} Along with public video datasets, we also chose some proprietary customer video datasets, which were captured at a traffic intersection and ran four different AUs i.e. pedestrian detection (PD), vehicle detection (VD), license plate detection (LPD) and license plate recognition (LPR). These AUs form the building blocks for Intelligent Transportation Systems (ITS) where high level AUs like accident prediction depend on accuracy of these low level AUs. 

%In this section, we show similar behavior i.e. optimal setting for one AU degrades accuracy for another AU.

\begin{table}[tb]
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline
    Setting & \multicolumn{4}{c|} {AU accuracy(\%)}\\
    \cline{2-5}
     & mAP$_{PD}$ & mAP$_{VD}$ & mAP$_{LPD}$  & acc$_{LPR}$ \\
    \hline
    \emph{PD-optimal} & 100.0 &  100.0 & 35.9 & 26.5\\
    \hline
    \emph{VD-optimal} & 98.6 & 100.0 & 37.1 & 24\\
    \hline
    \emph{LPD-optimal} & 99.6 & 99.2 & 42.0 & 25.9\\
    \hline
    \emph{LPR-optimal} & 100.0 & 100.0 & 36.4 & 33.4 \\
    \hline
\end{tabular}
\caption{Accuracy conflict for proprietary customer videos}
\label{tab:its-au}
 \vspace{-0.3in}
\end{table}

~\tabref{tab:its-au} shows the accuracy of these different AUs with different settings i.e. different optimal transformations being applied on the videos e.g. PD-optimal corresponds to the transformation setting that is optimal for PD, VD-optimal corresponds to the transformation setting that is optimal for VD, and so on. Accuracy for PD, VD and LPD is computed in terms of mAP using pycocotools~\cite{pycoco}. For LPR accuracy, we consider a license plate to be correctly recognized if and only if the IoU is greater than 0.6 and all characters in the license plate number are correctly recognized~\cite{xu2018towards}. We see that the accuracy for LPR with optimal settings for LPR is 33.4 \%, but this drops to 25.9 \%, 24 \% and 26.5 \% with LPD-optimal, VD-optimal and PD-optimal respectively. 

\textit{Thus, we see that even with pre-recorded videos, when we apply digital transformations (as a proxy to real camera settings change), we observe conflict in settings i.e. optimal setting for one AU degrades performance of another AU.}

%For PD, best transformation setting endeavours to increase the contrast, enhances the pixel intensity difference which in turn increases the distinguishability of person in the frame. While increasing contrast adds noise, which makes difficult for face-detection AU to detect small fine-grained features in faces, also shown in ~\figref{fig:impact-au-pics}. 

%Each point (x,y) in ~\figref{fig:impact-au} shows that (100-x)\% of video frames experience atleast a mAP degradation of y\%. ~\figref{fig:impact-au} shows both person-detection and face-detection AU suffer from accuracy degradation for significant number of frames when optimal transformation for a different AU is applied to augment the frames, also quantitatively presented in~\tabref{tab:retail}.

%Due to abundance and availability of pre-recorded videos, we first analyze the impact of camera parameter changes on pre-recorded videos for two different multi-tenant video analytics usecases. These public and customer videos are already captured with certain camera settings, hence we do not have the opportunity to change the real camera parameters and observe their impact. As an approximation, we apply different values of brightness, contrast, color-saturation and sharpness as a post-capture transformation using Python Imaging Library~\cite{pil} and then observe the impact of best transformation (i.e., provides highest AU accuracy) for one AU on accuracy of another AU insights in a multi-tenant video analytics system. 

%\paragraph{\textbf{Retail Store.}} We use two different AUs,  EfficientDet-v0~\cite{tan2020efficientdet} as person-detection AU and RetinaNet~\cite{deng2019retinaface} as face-detection AU to perform analytics on 13 video snippets from HMDB dataset~\cite{Kuehne11} and 8 video snippets from Olympics dataset~\cite{niebles2010modeling}. For both AU, derived insights are then compared with the ground-truths and we compute accuracy in terms of mean Average Precision (mAP) using pycocotools~\cite{pycoco}. 

%To apply various camera parameter setting on same scene content and to find the impact on analytical quality, we use proxies for the four camera parameters, also known as transformations~\cite{paul2021camtuner}. 

%For each of these detection AU, Algorithm~\ref{alg:det-conf-search} helps to find best transformation setting by employing a combination of mAP and true-positive IoU~\footnote{where single bounding box prediction for a object with IoU>0.5 with correct classification} as the analytical quality metric. Using Algorithm~\ref{alg:det-conf-search}, we find the best transformation setting (i.e., configuration) for face-detection (FD) and person-detection (PD) AU. In Algorithm~\ref{alg:impact-on-another}, we first apply digital augmentation on the frames extracted from video-snippet with these two best configurations and then obtain the difference in accuracy of the derived insights either by FD or by PD AU under those two transformation setting. ~\figref{fig:impact-au} indicates the fraction of frames that undergo in accuracy (i.e., mAP) degradation. Each point (x,y) in ~\figref{fig:impact-au} shows that (100-x)\% of video frames experience atleast a mAP degradation of y\%. ~\figref{fig:impact-au} shows both person-detection and face-detection AU suffer from accuracy degradation for significant number of frames when best transformation for a different AU is applied to augment the frames, also quantitatively presented in~\tabref{tab:retail}. 

%\textbf{Observation.} For person-detection AU, best transformation setting endeavours to increase the contrast, enhances the pixel intensity difference which in turn increases the distinguishability of person in the frame. While increasing contrast adds noise, which makes difficult for face-detection AU to detect small fine-grained features in faces, also shown in ~\figref{fig:impact-au-pics}. ~\figref{fig:impact-au} and~\tabref{tab:retail} both show that face-detection AU detecting small and finer features from face suffers from higher accuracy degradation than the coarse-grained person-detection AU.


%\paragraph{\textbf{Intelligent Transportation System (ITS).}} Usecase of ITS includes pedestrian detection (PD), vehicle detection (VD), license plate (LP) detection and recognition to enhance the road safety and traffic management. We use a object detector, i.e., efficientDet-v4~\cite{} as \emph{pedestrian} and \emph{vehicle} detection AU along with proprietary LP detection (LPD) and recognition(LPR) model from Neural labs~\cite{}. These AUs are then used to derive several insights from our customer video captured at a traffic junction.  Accuracy for derived insights by three detection AUs is computed in terms of mAP using pycocotools~\cite{pycoco}. We consider a LP is correctly recognized if and only if the IoU is greater than 0.6 and all characters in the LP number are correctly recognized~\cite{xu2018towards}.

%\begin{table}
%\begin{subtable}[h!]{0.45\textwidth}
%\centering
%\begin{tabular}{|c|c|c|c|c|}
%    \hline
%    Video-Dataset &  \multicolumn{4}{c|} {mAP degradation(\%)}\\
%    \cline{2-5}
%    & \multicolumn{2}{c|}{PD-bestConf for FD} & \multicolumn{2}{c|}{FD-bestConf for PD}\\
%    & \multicolumn{2}{c|}{(Impact on FD)} & \multicolumn{2}{c|}{(Impact on PD)}\\
%    \cline{2-3}\cline{4-5}
%    & Max & Mean & Max & Mean \\
%    \hline
%    HMDB51 & 100.0 & 20.89 & 73.42 & 15.32 \\
%    \hline
%    Olympics & 100.0 & 52.72 & 57.69 & 22.49 \\
%    \hline
%\end{tabular}
%\caption{Retail Store}
%\label{tab:retail}
%\end{subtable}
%\hfill
%\begin{subtable}[h!]{0.5\textwidth}
%\centering
%\begin{tabular}{|c|c|c|c|c|}
%    \hline
%    Best & \multicolumn{4}{c|} {AU accuracy(\%)}\\
%    \cline{2-5}
%    transformation & mAP$_{PD}$ & mAP$_{VD}$ & mAP$_{LPD}$  & acc$_{LPR}$ \\
%    \hline
%    \emph{PD} & 100.0 &  100.0 & 35.9 & 26.5\\
%    \hline
%    \emph{VD} & 98.6 & 100.0 & 37.1 & 24\\
%    \hline
%    \emph{LPD} & 99.6 & 99.2 & 42.0 & 25.9\\
%    \hline
%    \emph{LPR} & 100.0 & 100.0 & 36.4 & 33.4 \\
%    \hline
%\end{tabular}
%\caption{ITS}
%\label{tab:its-au}
%\end{subtable}
%\label{tab:impact-besttx}
%\caption{Impact of best transformation across AUs}
% \vspace{-0.3in}
%\end{table}

%\textbf{Observation.}~\tabref{tab:its-au} shows the accuracy variations of derived insights by different AUs under different AU-specific best transformations. The coarse-grained AUs i.e., person detection and vehicle detection AU do not exhibit performance variation under various AU-specific best transformation setting. But for the License plate recognition (LPR) that extracts fine-grained features, we observe significant accuracy degradation when best transformation for another AU is applied. For example, \emph{15} less license plates are correctly recognized when best transformation for vehicle detection is used to augment frames for LPR. 


%\paragraph{Different Camera Setting for different classes for same AU}
